Effective Abstract Reasoning with Dual-Contrast Network

As a step towards improving the abstract reasoning capability of machines, we aim to solve Raven's Progressive Matrices (RPM) with neural networks, since solving RPM puzzles is highly correlated with human intelligence. Unlike previous methods that use auxiliary annotations or assume hidden rules to produce appropriate feature representation, we only use the ground truth answer of each question for model learning, aiming for an intelligent agent to have a strong learning capability with a small amount of supervision. Based on the RPM problem formulation, the correct answer filled into the missing entry of the third row/column has to best satisfy the same rules shared between the first two rows/columns. Thus we design a simple yet effective Dual-Contrast Network (DCNet) to exploit the inherent structure of RPM puzzles. Specifically, a rule contrast module is designed to compare the latent rules between the filled row/column and the first two rows/columns; a choice contrast module is designed to increase the relative differences between candidate choices. Experimental results on the RAVEN and PGM datasets show that DCNet outperforms the state-of-the-art methods by a large margin of 5.77%. Further experiments on few training samples and model generalization also show the effectiveness of DCNet. Code is available at https://github.com/visiontao/dcnet.

==> fig_type.tex <==
\begin{figure*}[!t]
	\centering
	\includegraphics[width=1\textwidth]{figures/fig_type}
	\caption{Examples of 7 different figure configurations in the RAVEN dataset.}
	\label{fig_type}
\end{figure*}

==> sec_impact.tex <==
\section*{Broader Impact}
This work investigates the abstract reasoning capability of neural networks on RPM questions, which could help many research areas, including artificial intelligence, machine learning and computer vision. (1) RPM is highly correlated to human intelligence and it is based on logical rules. Thus solving RPM with machines can help to advance the general AI. (2) This work also helps the machine learning. As humans are able to solve RPM questions without intensive training and we hope machines could mimic this ability for efficient model learning. When few training samples are available, our model performs better on unseen problems and demonstrates good generalization ability. Therefore, our method can help to improve few-shot learning. (3) RPM question consists of images and the logical rules are manifested as visual structures. Since popular network architectures (\eg LSTM and ResNet) do not perform well on this task, solving RPM can help better understand and improve the contemporary computer vision systems.
